Hydropower optimization: an industrial approach

Nowadays hydroelectric energy is one of the best energy sources: it is cleaner, safer and more programmable than other sources. For this reason, its manage could not be done in an approssimative way, but advance mathematical models must be use. In this article we consider an overview of the problem: we introduce the problem, then we show its simplest but quite exaustive mathematical formulation and in the end we produce numerical results under the ipothesis that all input are deterministic.

==> case_study/Case_Study.tex <==
Let's move now to a real case study: this case, even though his semplicity, has all the elements that must be considered. 
Tagliamento hidroelectric site is situated is the north-east of Italy: on the top of the site there Lumiei lake and at the 
foot of it is there Ampezzo hydropower plant. Downstreamer,after two hours, water coming from Ampezzo flows into Lumiei lake
and then the water is used by Somplago power plant to produce electricity. At the end of its way, water emerges into Cavazzi lake.\\ 
Let's define now, the set of structural parameters that we need in our model, starting from the volumes of watersheed.\\
Let's state Lumiei whith label $1$ and Ambiesta with label $2$. Collection datas from $a2a$ company whe have:
\begin{align}
 V_{min}^1&=1,0677 \cdot 10^6 m^3,
 \nonumber\\
 V_{max}^1&=63,4364 \cdot 10^6 m^3, 
 \nonumber\\
 V_{min}^2&=0.4036 \cdot 10^6 m^3, 
 \nonumber\\
 V_{max}^2&=3.3507 \cdot 10^6 m^3.
 \nonumber
\end{align}
These are the structural parameters: fixed $i \in 1,\cdots,N$, generally it isn't requested that $V_{min,k}^i=V_{min}^i$, but it can happened that 
$V_{min,k}^i\ge V_{min}^i$, for some value of $k \in 1,\dots,N_h$ for some reason, such as landscape integrity. The same concept, reverse inequality, holds for basin maximum value. Anyway, we
consider $V_{min,k}^i=V_{min}^i$, $V_{max,k}^i=V_{max,k}^i$ for all $k=1,\cdots,N_h$: we consider later the values $V_{max,T}^i$ and $V_{min,T}^i$. We introduce
also a time of concentration $t_c=2$: water released from Lumiei lake takes two hours reach Ambiesta.\\
Let's move now to the hydropower station Ampezzo and Somplago. First of all we fix label $A$ for Ampezzo and $S$ for Somplago. Now, we need
to fix the maximum amount of water that coul be processed by the two hydropower plants.
\begin{align}
 T_{max}^A=15 \; \frac{m^3}{s}
 \nonumber\\
 T_{max}^S=75 \; \frac{m^3}{s}.
 \nonumber
\end{align}
As we observed before, in order to avoid an integer problem we fix $T_{max}^A=0 \; {m^3}/{s}$ and $T_{min}^S=0 \; {m^3}/{s}$. For the sake of semplicity,
as we have done for the volumes, we consider $T_{max,k}^j$ and $T_{min,k}^j$ constant in time, where $ j \in 1,\dots,M$ and $M$ is the number
of hydropower plants, in this case $M=2$. Than, the constraint about decision variables is, for example for Ampezzo plant, the following one
\begin{equation}
 T_{min}^A \le x_{k}^i \le T_{max}^A \quad i=1 \quad k=1,\dots,N_h
\nonumber
\end{equation}
\par Another important aspect is ho to model the energetic coefficient $K_e$: we have two choice: we can consider a constant $K_e$ and to do with
a linear optimization problem, or try to e more accurate and use a polynomial exprexion of height that leads to a non-linear objective function.\\
Experimental evidence show us that the second choice is better: indeed, the coefficient of Ambiesta and Somplago significantly changes relation
with the altitude of the lake. Denoting with $h$ the altitude of the lake we chose the following expressions for $K_e$ (mesured in 
$\frac{kWh}{m^3/s}$):
\begin{align}
 \begin{split}
 K_{e}^A= & -1.227 \cdot 10^{-9}h^4+4.288\cdot 10^{-7}h^3 -5.229 \cdot10^{-5}h^2 \\
          & + \cdot 4.170 \cdot 10^{-3}h+0.863370687,
 \nonumber\\
 K_{e}^S= &-1.937 \cdot 10^{-4}h^4+2.206\cdot 10^{-3}h^3 -1.032 \cdot10^{-2}h^2\\
         & + \cdot 3.230 \cdot 10^{-2}h+0.60914.
 \nonumber 
 \end{split}
 \end{align}
\par Let's see now, how we can impose volumes constraints. We have observed that $V_{min,k}^i \le V_{k}^i \le V_{max,k}^i$ for $i=1,\dots,N$ and 
for $k=1,\dots,N_h$. It is clear that the volume $V_{k}^i$ is function of the decision variables $x_{l}^i$ for $l\le i$: indeed, the reservoir
at time $i$ is affect by the amount of water used in the past. Moreover, watershed volume depends by the tributary discharges in the past, from the 
beginning to the present istant $i$. We model all the tributary flows as a single function $a\left(t\right)^i$ that contains all hydro flows to the
basin $i$. Considering a discrete greed of times, we have a deterministic sequence of hydro contributions $a_{k}^i$.\\
Denoting whit $V_{0}^i$ catch basin starting volume, a minimum volume constrain can be written in the following way:
\begin{equation}
 V_{k}^i = V_{0}^i + \sum_{l=1}^{k} a_{l}^i - \sum_{l=1}^{k} x_{l}^i \ge V_{min,k}^i.
\label{label_volume_equation}
\end{equation}
It is also important to note that if watershed $i$ is linked to watershed $j$ which pours water in basin $i$ then  constraint $\eqref{label_volume_equation}$
must be rewritten as follows:
\begin{equation}
 V_{k}^i = V_{0}^i + \sum_{l=1}^{k} a_{l}^i - \sum_{l=1}^{k} x_{l}^i + \sum_{l=1}^{k - t_c} x_{l}^j \ge V_{min,k}^i.
\nonumber
\end{equation}
where $t_c$ is concentration time, suppose to be an integer multiple of $\Delta h$. In case not, fractional amount of water
relased from $j$ at times $k -\left\lceil t_c \right\rceil$ and $k-\left\lfloor t_c \right\rfloor$ must be considered, as staded above.
\par Another tipe of constraint that must be considered is about the decision variables. As we said above, $x_{k}^i$ is such that
\begin{equation}
 T_{min,k}^i \le x_{k}^i \le T_{max,k}^i, \quad i=1,\dots,N. \quad k=1,\dots,N_h,
 \nonumber
\end{equation}
that in this specific case becomes:
\begin{equation}
 0 \le x_{k}^i \le T_{max}^i, \quad i=1,\dots,N.
 \nonumber
\end{equation}
\par Considering a given price forecast, stated with $P_{k}$ for $k=1,\dots,N_h$, our objective function $f$ is:
\begin{equation}
\max_{\boldsymbol{x}}  \sum_{k=1}^{N_h} \sum_{i=1}^N \sum_{j \in down_i} Ke_j \left(h_{k}^i,k\right) x_{k}^i P_k.
\end{equation}
In this formulation, we didn't considered the spilling: we briefly debate about it later.

\subsection{Numeric results}
It this section we consider three different scenarios. The first scenario could be considered as a standard case. We have a normal flows profile
and a given price forecast. The input variables are shown in Table $\eqref{Tabella_input_Scenario_1}$.

\begin{table}
\centering
\begin{tabular}{ccc}
\toprule
$P_z$ 	  & $a^1$     & $a^2$\\
$EUR$     & $m^3/s$   & $m^3/s$\\
\midrule
62.20 & 2.4000 & 11.5040 \\ 
54.49 & 2.4000 & 11.5037 \\ 
52.57 & 2.4000 & 11.5033ì \\ 
52.40 & 2.4000 & 11.5030 \\ 
50.33 & 2.4000 & 11.5026 \\ 
52.81 & 2.3000 & 11.3023 \\ 
65.38 & 2.3000 & 11.3019 \\ 
67.75 & 2.3000 & 11.3016 \\ 
73.99 & 2.3000 & 11.2012 \\ 
69.99 & 2.3000 & 11.2009 \\ 
64.26 & 2.3000 & 11.2005 \\ 
62.37 & 2.3000 & 11.2002 \\ 
55.34 & 2.3000 & 11.1998 \\ 
55.27 & 2.3000 & 11.1995 \\ 
59.05 & 2.3000 & 11.1992 \\ 
59.41 & 2.3000 & 11.1989 \\ 
62.49 & 2.3000 & 11.1986 \\ 
66.40 & 2.3000 & 11.1982 \\ 
82.33 & 2.3000 & 11.1979 \\ 
73.29 & 2.3000 & 11.1976 \\ 
64.35 & 2.3000 & 11.1973 \\ 
62.88 & 2.3000 & 11.1970 \\ 
62.40 & 2.3000 & 11.1966 \\ 
55.99 & 2.3000 & 11.1963 \\ 
\bottomrule
\end{tabular}
\caption{Input values for the first scenario}
\label{Tabella_input_Scenario_1}
\end{table}
Then we have to set the starting and the final value of the two watershed. Let's state:
\begin{align}
V_{0}^1= 25 \cdot 10^6 \; m^3,\\
\nonumber 
V_{T}^1= 25 \cdot 10^6 \; m^3,\\
\nonumber
V_{0}^2= 2.8 \cdot 10^6 \; m^3,\\
\nonumber
V_{T}^2= 2.8 \cdot 10^6 \; m^3.
\nonumber
\end{align}
In real cases it is common to set the starting and the ending value to be equal.
Considering these inputs and the parameters in the previous section, after the optimization process, we have the following results in Table 
$\eqref{Tabella_output_Scenario_1}$.

\begin{table}
\centering
\begin{tabular}{ccc}
\toprule
$P_z$ 	  & $T^A$     & $T^S$\\
$EUR$     & $m^3/s$   & $m^3/s$\\
\midrule
62.20 & 0.0000 & 0.0000 \\ 
54.49 & 0.0000 & 0.0000 \\ 
52.57 & 0.0000 & 0.0000 \\ 
52.40 & 0.0000 & 0.0000 \\ 
50.33 & 0.0000 & 0.0000 \\ 
52.81 & 0.0000 & 0.0000 \\ 
65.38 & 0.0000 & 0.0000 \\ 
67.75 & 0.0000 & 26.3011 \\ 
73.99 & 15.0000 & 75.0000 \\ 
69.99 & 10.6998 & 75.0000 \\ 
64.26 & 0.0000 & 0.0000 \\ 
62.37 & 0.0000 & 0.0000 \\ 
55.34 & 0.0000 & 0.0000 \\ 
55.27 & 0.0000 & 0.0000 \\ 
59.05 & 0.0000 & 0.0000 \\ 
59.41 & 0.0000 & 0.0000 \\ 
62.49 & 0.0000 & 0.0000 \\ 
66.40 & 0.0000 & 0.0000 \\ 
82.33 & 15.0000 & 75.0000 \\ 
73.29 & 15.0000 & 75.0000 \\ 
64.35 & 0.0000 & 0.0000 \\ 
62.88 & 0.0000 & 0.0000 \\ 
62.40 & 0.0000 & 0.0000 \\ 
55.99 & 0.0000 & 0.0000 \\ 
\bottomrule
\end{tabular}
\caption{Results of the first scenario.}
\label{Tabella_output_Scenario_1}
\end{table}

As we can see from these results and from Figure $\eqref{Production_Scenario_1}$ , it is clear that the production of energy is concentrated where electricity price are heighter.
In Figure $\eqref{Volumes_Scenario_1}$ gate volumes is shown: it is clear from this figure that all constraints about volumes are hourly fullfilled.
\begin{figure}[!ht]
\centering
\begin{subfigure}[Prices and flows]
  {
  \includegraphics[scale=0.5]{./Case_Study/Scenarios/Scenario_1/Power_Prices_Scen1.eps}
  \label{Production_Scenario_1}
  }
\end{subfigure}
\begin{subfigure}[Volumes]
  {
  \includegraphics[scale=0.5]{./Case_Study/Scenarios/Scenario_1/Volumes_Scen1.eps}
  \label{Volumes_Scenario_1}
  }
\end{subfigure}
\caption{As observed before, the production concentrated where prices are heigher while all constrants are satisfied.}
\end{figure}


\subsubsection{A inflows shortage}
Let's consider now another type of situation. In this case, as is shown in Table $\eqref{Tabella_input_Scenario_2}$, no incoming
flows are present: neither in Lumiei nor Ambiesta.
Let's set the following volumes:
\begin{align}
V_{0}^1= 24 \cdot 10^6 \; m^3,\\
\nonumber 
V_{T}^1= 23 \cdot 10^6 \; m^3,\\
\nonumber
V_{0}^2= 2 \cdot 10^6 \; m^3,\\
\nonumber
V_{T}^2= 3 \cdot 10^6 \; m^3.
\nonumber
\end{align}
We expect that Ampezzo will start producing energy to supply water to downstream watershed of Ambista, that must reach the minimum volume
of $V_{T}^2= 3 \cdot 10^6 \; m^3$ by the end of the day. Moreover, it's rational to suppose that Somplago will minimize its production
in order to avoid waste water. From the results is Table $\eqref{Tabella_output_Scenario_2}$ and Figure $Production_Scenario_2$ we observe
that actually this is what happens. Moreover, from Figure ${Volumes_Scenario_2}$, we observe that volumes constraint are all satisfied and
that, at the end of the day, Ambiesta valley reaches the wanted final value.

\begin{table}
\centering
\begin{tabular}{ccc}
\toprule
$P_z$ 	  & $a^1$     & $a^2$\\
$EUR$     & $m^3/s$   & $m^3/s$\\
\midrule
95.0000 & 0.0000 & 0.0000 \\ 
85.0000 & 0.0000 & 0.0000 \\ 
90.0000 & 0.0000 & 0.0000 \\ 
52.4000 & 0.0000 & 0.0000 \\ 
50.3300 & 0.0000 & 0.0000 \\ 
52.8100 & 0.0000 & 0.0000 \\ 
65.3800 & 0.0000 & 0.0000 \\ 
67.7500 & 0.0000 & 0.0000 \\ 
73.9900 & 0.0000 & 0.0000 \\ 
69.9900 & 0.0000 & 0.0000 \\ 
64.2600 & 0.0000 & 0.0000 \\ 
62.3700 & 0.0000 & 0.0000 \\ 
55.3400 & 0.0000 & 0.0000 \\ 
55.2700 & 0.0000 & 0.0000 \\ 
59.0500 & 0.0000 & 0.0000 \\ 
59.4100 & 0.0000 & 0.0000 \\ 
62.4900 & 0.0000 & 0.0000 \\ 
66.4000 & 0.0000 & 0.0000 \\ 
82.3300 & 0.0000 & 0.0000 \\ 
73.2900 & 0.0000 & 0.0000 \\ 
64.3500 & 0.0000 & 0.0000 \\ 
62.8800 & 0.0000 & 0.0000 \\ 
62.4000 & 0.0000 & 0.0000 \\ 
55.9900 & 0.0000 & 0.0000 \\ 

\bottomrule
\end{tabular}
\caption{Input values for the second scenario}
\label{Tabella_input_Scenario_2}
\end{table}

\begin{table}
\centering
\begin{tabular}{ccc}
\toprule
$P_z$ 	  & $T^A$     & $T^S$\\
$EUR$     & $m^3/s$   & $m^3/s$\\
\midrule
95.0000 & 15.0000 & 0.0000 \\ 
85.0000 & 15.0000 & 0.0000 \\ 
90.0000 & 15.0000 & 0.0000 \\ 
52.4000 & 0.0000 & 0.0000 \\ 
50.3300 & 0.0000 & 0.0000 \\ 
52.8100 & 0.0000 & 0.0000 \\ 
65.3800 & 15.0000 & 0.0000 \\ 
67.7500 & 15.0000 & 0.0000 \\ 
73.9900 & 15.0000 & 0.0000 \\ 
69.9900 & 15.0000 & 0.0000 \\ 
64.2600 & 15.0000 & 0.0000 \\ 
62.3700 & 15.0000 & 0.0000 \\ 
55.3400 & 15.0000 & 0.0000 \\ 
55.2700 & 7.7881 & 0.0000 \\ 
59.0500 & 15.0000 & 0.0000 \\ 
59.4100 & 15.0000 & 0.0000 \\ 
62.4900 & 15.0000 & 0.0000 \\ 
66.4000 & 15.0000 & 0.0000 \\ 
82.3300 & 15.0000 & 0.0000 \\ 
73.2900 & 15.0000 & 0.0000 \\ 
64.3500 & 15.0000 & 0.0000 \\ 
62.8800 & 15.0000 & 0.0000 \\ 
62.4000 & 0.0000 & 0.0000 \\ 
55.9900 & 0.0000 & 0.0000 \\ 
\bottomrule
\end{tabular}
\caption{Results of the second scenario.}
\label{Tabella_output_Scenario_2}
\end{table}

\begin{figure}[!ht]
\centering
\begin{subfigure}[Prices and flows]
  {
  \includegraphics[scale=0.5]{./Case_Study/Scenarios/Scenario_2/Power_Prices_Scen2.eps}
  \label{Production_Scenario_2}
  }
\end{subfigure}
\begin{subfigure}[Volumes]
  {
  \includegraphics[scale=0.5]{./Case_Study/Scenarios/Scenario_2/Volumes_Scen2.eps}
  \label{Volumes_Scenario_2}
  }
\end{subfigure}
\caption{Ampezzo increases its production to supply water to Ambiesta that reaches the desidered final value of $3 \cdot 10^6 \; m^3$ }
\end{figure}

\subsubsection{A inflows profusion}
Let's consider now a different situation. Suppose that the day is particulary rainy and that the two basin starting level is quite hight. It
can happen that not all the water could be used to produce energy and so, to avoid a disaster due to lake overflow, we must spill away some water
when we are near to the maximum reservoir level. Consider inputs in Table $\eqref{Tabella_input_Scenario_3}$ and the following starting volumes 
\begin{align}
V_{0}^1= 63.4364 \cdot 10^6 \; m^3,\\
\nonumber 
V_{T}^1= 63 \cdot 10^6 \; m^3,\\
\nonumber
V_{0}^2= 3 \cdot 10^6 \; m^3,\\
\nonumber
V_{T}^2= 2 \cdot 10^6 \; m^3.
\nonumber
\end{align}
Let's suppose, in addiction, that 
\begin{align}
 T_{max}^A=16 \; \frac{m^3}{s}
 \nonumber\\
 T_{max}^S=75 \; \frac{m^3}{s},
 \nonumber
\end{align}
and, in order to have a linear model, suppose that $K_e$ coefficients are constant. In particular we state: $k_{e}^A=$ and $K_{e}^S=$.
\par As state before, where a spill is ammissible, volumes constraints and objective function must be modified. We state with $y_{i}^1$ the 
amount of water spilled away from watershed $1$ at time $i$.
Generally speaking, volume constraint for a generic basin at time $n$ will have the following formulation
\begin{equation}
 V_{i}^1=V_{0}^1-\sum_{i=1}^{n}x_{i}^1 - \sum_{i=1}^n y_{i}^1 + \sum_{i=1}^n a_{i}^1 \le V_{max,n}^1.
 \nonumber
\end{equation}
Constrain for minimum volume is simular.
\par As we discussed, objective function have to be modified adding a penalization term that consider the possibility of splilling water away. 
If we consider the linear case and our particular problem, one possibility is the following one:

\begin{equation}
\max_{\boldsymbol{x},\boldsymbol{y}}  \sum_{k=1}^{N_h} \sum_{i=1}^N \sum_{j \in down_i} Ke_j x_{k}^i P_k - Ke_j y_{k}^i P_k.
\end{equation}
When the solver try to solve the optimization problem maximizing the objective function, it tries to minimize the negative term: subsequently
the spilled water is minimized and this is exactly what we exprect because throw water away causes an econimic damage, and this must be avoid. 
Consider the input flows and a price forecast shown in Table $\eqref{Tabella_input_Scenario_3}$.

\begin{table}
\centering
\begin{tabular}{ccc}
\toprule
$P_z$ 	  & $a^1$     & $a^2$\\
$EUR$     & $m^3/s$   & $m^3/s$\\
\midrule
62.20 & 3.8939 & 6.8142 \\ 
54.49 & 2.3661 & 10.2112 \\ 
52.57 & 26.6213 & 17.9784 \\ 
52.40 & 10.8930 & 0.3026 \\ 
50.33 & 28.6057 & 4.6058 \\ 
52.81 & 5.4198 & 13.3490 \\ 
65.38 & 15.0905 & 14.8075 \\ 
67.75 & 8.3589 & 16.2404 \\ 
73.99 & 27.1316 & 9.5660 \\ 
69.99 & 0.2631 & 15.3093 \\ 
64.26 & 19.3790 & 8.9293 \\ 
62.37 & 8.6549 & 14.8768 \\ 
55.34 & 14.0189 & 6.5074 \\ 
55.27 & 12.3195 & 18.8859 \\ 
59.05 & 8.8246 & 6.4141 \\ 
59.41 & 3.6650 & 15.3259 \\ 
62.49 & 14.2966 & 12.0654 \\ 
66.40 & 17.6182 & 2.7215 \\ 
82.33 & 1.0162 & 17.4639 \\ 
73.29 & 10.3653 & 8.3677 \\ 
64.35 & 32.8793 & 13.2517 \\ 
62.88 & 1.4572 & 13.6735 \\ 
62.40 & 10.1707 & 0.5120 \\ 
55.99 & 13.5839 & 12.5866 \\ 
\bottomrule
\end{tabular}
\caption{Input values for the third scenario}
\label{Tabella_input_Scenario_3}
\end{table}

We have the following results:
\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
$P_z$ 	  & $T^A$     & $T^S$   & $Spill^1$ & $Spill^2$\\
$EUR$     & $m^3/s$   & $m^3/s$ & $m^3/s$   & $m^3/s$ \\
\midrule
62.20 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
54.49 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
52.57 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
52.40 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
50.33 & 8.3800 & 75.0000 & 0.0000 & 150.7162 \\ 
52.81 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
65.38 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
67.75 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
73.99 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
69.99 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
64.26 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
62.37 & 2.3167 & 75.0000 & 0.0000 & 0.0000 \\ 
55.34 & 0.0000 & 75.0000 & 0.0000 & 200.0000 \\ 
55.27 & 16.0000 & 75.0000 & 0.0000 & 200.0000 \\ 
59.05 & 16.0000 & 75.0000 & 0.0000 & 115.6778 \\ 
59.41 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
62.49 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
66.40 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
82.33 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
73.29 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
64.35 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
62.88 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
62.40 & 16.0000 & 75.0000 & 0.0000 & 0.0000 \\ 
55.99 & 16.0000 & 15.1624 & 0.0000 & 0.0000 \\ 
\bottomrule
\end{tabular}
\caption{Results of the third scenario.}
\label{Tabella_output_Scenario_3}
\end{table}

Looking at results in Table $\eqref{Tabella_output_Scenario_3}$ and in Figure $\eqref{Figure_Scenario_3}$ we notice that the maximum quantity
of whater that is thrown away occurs when prices are lower. This is quite intuitive, but only because the problem is linear. Indeed, it might be more
appropriate trowing away water in other periods if $K_e$ depends by the level of the basin. For example it could be smarter to conserve water
when prices are low in order to reach an higher level improving the efficiency of the turbine, so that we can produce more energy with the same
amount of water. Anyway, all these consideration hinge on a lot of factor such as energetic coefficient expression, energy prices outline ans so
on.\\
We can also observe in $\eqref{Volumes_Scenario_3}$ that all volumes constraints are satisfied, thanks to the spill possibility. Indeed, without
the variable $\boldsymbol{y}$ the problem would be infeasible becaus volumes constraints would never been respected.
  
  
\begin{figure}[!ht]
\centering
\begin{subfigure}[Prices and flows]
  {
  \includegraphics[scale=0.6]{./Case_Study/Scenarios/Scenario_3/Power_Prices_Scen3.eps}
  \label{Production_Scenario_3}
  }
\end{subfigure}
\begin{subfigure}[Volumes]
  {
  \includegraphics[scale=0.6]{./Case_Study/Scenarios/Scenario_3/Volumes_Scen3.eps}
  \label{Volumes_Scenario_3}
  }
\end{subfigure}
\caption{Volumes and producions for the third scenario.}
\label{Figure_Scenario_3}
\end{figure}
